Diffusion Models for Constrained Domains

Denoising diffusion models are a novel class of generative algorithms that achieve state-of-the-art performance across a range of domains, including image generation and text-to-image tasks. Building on this success, diffusion models have recently been extended to the Riemannian manifold setting, broadening their applicability to a range of problems from the natural and engineering sciences. However, these Riemannian diffusion models are built on the assumption that their forward and backward processes are well-defined for all times, preventing them from being applied to an important set of tasks that consider manifolds defined via a set of inequality constraints. In this work, we introduce a principled framework to bridge this gap. We present two distinct noising processes based on (i) the logarithmic barrier metric and (ii) the reflected Brownian motion induced by the constraints. As existing diffusion model techniques cannot be applied in this setting, we derive new tools to define such models in our framework. We then demonstrate the practical utility of our methods on a number of synthetic and real-world tasks, including applications from robotics and protein design.

==> sections/ackn.tex <==
\section*{Software and data}

The core set of tools in Python \citep{van1995python} enabled this work, including Jax \citep{jax2018github}, Optax \citep{deepmind2020jax}, Haiku \citep{haiku2020github}, Hydra \citep{Yadan2019Hydra}, Numpy \citep{harris2020}, Scipy \citep{2020SciPy-NMeth} and Matplotlib \citep{Hunter2007}.

% \section*{Acknowledgements}

% We thank the anonymous reviewers for their insightful and constructive comments. AP and MH are funded through the StatML CDT through grant EP/S023151/1. AD acknowledges support of the UK Defence Science and Technology Laboratory (Dstl) and Engineering and Physical Research Council (EPSRC) under grant EP/R013616/1. This is part of the collaboration between US DOD, UK MOD and UK EPSRC under the Multidisciplinary University Research Initiative. AD is also partially supported by the EPSRC grant EP/R034710/1 CoSines.
% EM is supported by an EPSRC Prosperity Partnership EP/T005386/1 between Microsoft Research and the University of Cambridge.


